Spatial CAPTCHA: Generatively Benchmarking Spatial Reasoning for Human-Machine Differentiation

Online services rely on CAPTCHAs as a first line of defense against automated abuse, yet recent advances in multi-modal large language models (MLLMs) have eroded the effectiveness of conventional designs that focus on text recognition or 2D image understanding. To address this challenge, we present Spatial CAPTCHA, a novel human-verification framework that leverages fundamental differences in spatial reasoning between humans and MLLMs. Unlike existing CAPTCHAs which rely on low-level perception tasks that are vulnerable to modern AI, Spatial CAPTCHA generates dynamic questions requiring geometric reasoning, perspective-taking, occlusion handling, and mental rotation. These skills are intuitive for humans but difficult for state-of-the-art (SOTA) AI systems. The system employs a procedural generation pipeline with constraint-based difficulty control, automated correctness verification, and human-in-the-loop validation to ensure scalability, robustness, and adaptability. Evaluation on a corresponding benchmark, Spatial-CAPTCHA-Bench, demonstrates that humans vastly outperform 10 state-of-the-art MLLMs, with the best model achieving only 31.0% Pass@1 accuracy. Furthermore, we compare Spatial CAPTCHA with Google reCAPTCHA, which confirms its effectiveness as both a security mechanism and a diagnostic tool for spatial reasoning in AI.

==> Figures/fig_answer_response_times.tex <==
\begin{figure*}[b!]
\vspace{-1.5em}
\scriptsize
\centering
\begin{subfigure}{0.5\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    boxplot/draw direction = y,
    ymode=log,
    width=8cm,
    height=7.0cm,
    ylabel={Response Time [s]},
    xtick={1,...,10},
    xticklabels={
        opus-4,
        sonnet-4,
        gemini-2.5-flash,
        gemini-2.5-pro,
        llama-4-maverick,
        phi-4-multimodal,
        mistral-medium-3,
        chatgpt-4o,
        o4-mini,
        qwen2.5-vl-72b,
    },
    xticklabel style={rotate=60, anchor=north east, font=\small},
    ymin=0.3, ymax=353.6,
    axis x line=bottom,
    axis y line=left,
    boxplot/variable width,
    enlarge x limits=0.05,
    line width=1pt,
    every boxplot/.append style={thick},
]

\definecolor{myred}{RGB}{230,97,1}
\definecolor{myorange}{RGB}{253,184,99}
\definecolor{mybrown}{RGB}{178,171,210}
\definecolor{mygreen}{RGB}{120,198,121}
\definecolor{myteal}{RGB}{27,158,119}
\definecolor{myblue}{RGB}{66,146,198}
\definecolor{mypurple}{RGB}{158,154,200}
\definecolor{mycyan}{RGB}{102,194,165}

\addplot+[
    boxplot prepared={lower whisker=2.16, lower quartile=7.69, median=9.95, upper quartile=12.01, upper whisker=18.47},
    fill=blue!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=1.52, lower quartile=2.72, median=3.31, upper quartile=3.97, upper whisker=5.84},
    fill=red!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=1.16, lower quartile=1.57, median=1.81, upper quartile=2.22, upper whisker=3.20},
    fill=green!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=7.21, lower quartile=17.56, median=95.38, upper quartile=160.47, upper whisker=321.49},
    fill=orange!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=0.35, lower quartile=0.92, median=1.17, upper quartile=1.81, upper whisker=3.13},
    fill=purple!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=0.63, lower quartile=1.19, median=1.54, upper quartile=2.03, upper whisker=3.28},
    fill=brown!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=0.86, lower quartile=1.46, median=1.78, upper quartile=2.13, upper whisker=3.12},
    fill=pink!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=0.92, lower quartile=1.50, median=1.90, upper quartile=2.46, upper whisker=3.90},
    fill=olive!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=10.40, lower quartile=44.33, median=65.27, upper quartile=94.85, upper whisker=170.62},
    fill=cyan!20, draw=black
] coordinates {};

\addplot[
    boxplot prepared={lower whisker=0.90, lower quartile=1.46, median=1.82, upper quartile=2.66, upper whisker=4.47},
    fill=magenta!20, draw=black
] coordinates {};

\end{axis}
\end{tikzpicture}
\caption{Answer time by model}
\label{fig:Time-by-Model}
\end{subfigure}%
\hfill
\begin{subfigure}{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.24]
    \coordinate (origin) at (0, 0);

    \def\maxscale{10}

    \foreach[count=\i] \dim in {Agent Sight, Full Views, Polyomino, Pyramid, Revolution, Sun Direction, Unfolded}{
        \draw[gray!50] (origin) -- (\i * 360 / 7: \maxscale);
        \node (title) at (\i * 360 / 7: 11) {\small\dim};

        \foreach \r in {2,4,6,8,10}{
            \draw[gray!30, very thin] (\i * 360 / 7: \r) arc (\i * 360 / 7:\i * 360 / 7 + 360/7:\r);
        }
    }

    \foreach \r in {2,4,6,8,10}{
        \draw[gray!30, dotted] (0,0) circle (\r);
    }

    \coordinate (p0_1) at (1 * 360 / 7: 0.0);
    \coordinate (p0_2) at (2 * 360 / 7: 2.5);
    \coordinate (p0_3) at (3 * 360 / 7: 0.8);
    \coordinate (p0_4) at (4 * 360 / 7: 0.5);
    \coordinate (p0_5) at (5 * 360 / 7: 0.1);
    \coordinate (p0_6) at (6 * 360 / 7: 1.1);
    \coordinate (p0_7) at (7 * 360 / 7: 0.0);

    \draw[thick, blue, fill=blue!20, opacity=.7] (p0_1) -- (p0_2) -- (p0_3) -- (p0_4) -- (p0_5) -- (p0_6) -- (p0_7) -- cycle;

    \draw[fill=blue!20, opacity=.7] (-10,-15) rectangle (-9,-14);
    \node[anchor=west] at (-8.5,-14.5) {\footnotesize opus-4};

    \coordinate (p1_1) at (1 * 360 / 7: 1.2);
    \coordinate (p1_2) at (2 * 360 / 7: 2.4);
    \coordinate (p1_3) at (3 * 360 / 7: 2.9);
    \coordinate (p1_4) at (4 * 360 / 7: 2.4);
    \coordinate (p1_5) at (5 * 360 / 7: 2.0);
    \coordinate (p1_6) at (6 * 360 / 7: 3.1);
    \coordinate (p1_7) at (7 * 360 / 7: 1.0);

    \draw[thick, red, fill=red!20, opacity=.7] (p1_1) -- (p1_2) -- (p1_3) -- (p1_4) -- (p1_5) -- (p1_6) -- (p1_7) -- cycle;

    \draw[fill=red!20, opacity=.7] (-10,-17) rectangle (-9,-16);
    \node[anchor=west] at (-8.5,-16.5) {\footnotesize sonnet-4};

    \coordinate (p2_1) at (1 * 360 / 7: 2.1);
    \coordinate (p2_2) at (2 * 360 / 7: 3.1);
    \coordinate (p2_3) at (3 * 360 / 7: 2.1);
    \coordinate (p2_4) at (4 * 360 / 7: 1.7);
    \coordinate (p2_5) at (5 * 360 / 7: 2.3);
    \coordinate (p2_6) at (6 * 360 / 7: 2.9);
    \coordinate (p2_7) at (7 * 360 / 7: 1.0);

    \draw[thick, green, fill=green!20, opacity=.7] (p2_1) -- (p2_2) -- (p2_3) -- (p2_4) -- (p2_5) -- (p2_6) -- (p2_7) -- cycle;

    \draw[fill=green!20, opacity=.7] (-10,-19) rectangle (-9,-18);
    \node[anchor=west] at (-8.5,-18.5) {\footnotesize gemini-2.5-flash};

    \coordinate (p3_1) at (1 * 360 / 7: 2.9);
    \coordinate (p3_2) at (2 * 360 / 7: 2.4);
    \coordinate (p3_3) at (3 * 360 / 7: 2.3);
    \coordinate (p3_4) at (4 * 360 / 7: 4.4);
    \coordinate (p3_5) at (5 * 360 / 7: 3.4);
    \coordinate (p3_6) at (6 * 360 / 7: 3.4);
    \coordinate (p3_7) at (7 * 360 / 7: 1.4);

    \draw[thick, orange, fill=orange!20, opacity=.7] (p3_1) -- (p3_2) -- (p3_3) -- (p3_4) -- (p3_5) -- (p3_6) -- (p3_7) -- cycle;

    \draw[fill=orange!20, opacity=.7] (-10,-21) rectangle (-9,-20);
    \node[anchor=west] at (-8.5,-20.5) {\footnotesize gemini-2.5-pro};

    \coordinate (p4_1) at (1 * 360 / 7: 2.7);
    \coordinate (p4_2) at (2 * 360 / 7: 2.9);
    \coordinate (p4_3) at (3 * 360 / 7: 2.1);
    \coordinate (p4_4) at (4 * 360 / 7: 1.3);
    \coordinate (p4_5) at (5 * 360 / 7: 2.1);
    \coordinate (p4_6) at (6 * 360 / 7: 3.1);
    \coordinate (p4_7) at (7 * 360 / 7: 0.9);

    \draw[thick, purple, fill=purple!20, opacity=.7] (p4_1) -- (p4_2) -- (p4_3) -- (p4_4) -- (p4_5) -- (p4_6) -- (p4_7) -- cycle;

    \draw[fill=purple!20, opacity=.7] (-10,-23) rectangle (-9,-22);
    \node[anchor=west] at (-8.5,-22.5) {\footnotesize llama-4-maverick};

    \coordinate (p5_1) at (1 * 360 / 7: 2.6);
    \coordinate (p5_2) at (2 * 360 / 7: 2.0);
    \coordinate (p5_3) at (3 * 360 / 7: 2.3);
    \coordinate (p5_4) at (4 * 360 / 7: 1.9);
    \coordinate (p5_5) at (5 * 360 / 7: 2.2);
    \coordinate (p5_6) at (6 * 360 / 7: 2.9);
    \coordinate (p5_7) at (7 * 360 / 7: 1.9);

    \draw[thick, brown, fill=brown!20, opacity=.7] (p5_1) -- (p5_2) -- (p5_3) -- (p5_4) -- (p5_5) -- (p5_6) -- (p5_7) -- cycle;

    \draw[fill=brown!20, opacity=.7] (2,-15) rectangle (3,-14);
    \node[anchor=west] at (3.5,-14.5) {\footnotesize phi-4-multimodal};

    \coordinate (p6_1) at (1 * 360 / 7: 3.0);
    \coordinate (p6_2) at (2 * 360 / 7: 2.1);
    \coordinate (p6_3) at (3 * 360 / 7: 2.4);
    \coordinate (p6_4) at (4 * 360 / 7: 1.4);
    \coordinate (p6_5) at (5 * 360 / 7: 1.6);
    \coordinate (p6_6) at (6 * 360 / 7: 2.5);
    \coordinate (p6_7) at (7 * 360 / 7: 1.1);

    \draw[thick, pink, fill=pink!20, opacity=.7] (p6_1) -- (p6_2) -- (p6_3) -- (p6_4) -- (p6_5) -- (p6_6) -- (p6_7) -- cycle;

    \draw[fill=pink!20, opacity=.7] (2,-17) rectangle (3,-16);
    \node[anchor=west] at (3.5,-16.5) {\footnotesize mistral-medium-3};

    \coordinate (p7_1) at (1 * 360 / 7: 2.2);
    \coordinate (p7_2) at (2 * 360 / 7: 3.5);
    \coordinate (p7_3) at (3 * 360 / 7: 1.9);
    \coordinate (p7_4) at (4 * 360 / 7: 4.4);
    \coordinate (p7_5) at (5 * 360 / 7: 2.7);
    \coordinate (p7_6) at (6 * 360 / 7: 2.5);
    \coordinate (p7_7) at (7 * 360 / 7: 1.1);

    \draw[thick, olive, fill=olive!20, opacity=.7] (p7_1) -- (p7_2) -- (p7_3) -- (p7_4) -- (p7_5) -- (p7_6) -- (p7_7) -- cycle;

    \draw[fill=olive!20, opacity=.7] (2,-19) rectangle (3,-18);
    \node[anchor=west] at (3.5,-18.5) {\footnotesize chatgpt-4o};

    \coordinate (p8_1) at (1 * 360 / 7: 2.8);
    \coordinate (p8_2) at (2 * 360 / 7: 2.1);
    \coordinate (p8_3) at (3 * 360 / 7: 3.0);
    \coordinate (p8_4) at (4 * 360 / 7: 6.0);
    \coordinate (p8_5) at (5 * 360 / 7: 2.1);
    \coordinate (p8_6) at (6 * 360 / 7: 4.3);
    \coordinate (p8_7) at (7 * 360 / 7: 1.3);

    \draw[thick, cyan, fill=cyan!20, opacity=.7] (p8_1) -- (p8_2) -- (p8_3) -- (p8_4) -- (p8_5) -- (p8_6) -- (p8_7) -- cycle;

    \draw[fill=cyan!20, opacity=.7] (2,-21) rectangle (3,-20);
    \node[anchor=west] at (3.5,-20.5) {\footnotesize o4-mini};

    \coordinate (p9_1) at (1 * 360 / 7: 1.7);
    \coordinate (p9_2) at (2 * 360 / 7: 3.1);
    \coordinate (p9_3) at (3 * 360 / 7: 2.6);
    \coordinate (p9_4) at (4 * 360 / 7: 3.5);
    \coordinate (p9_5) at (5 * 360 / 7: 1.7);
    \coordinate (p9_6) at (6 * 360 / 7: 2.9);
    \coordinate (p9_7) at (7 * 360 / 7: 1.3);

    \draw[thick, magenta, fill=magenta!20, opacity=.7] (p9_1) -- (p9_2) -- (p9_3) -- (p9_4) -- (p9_5) -- (p9_6) -- (p9_7) -- cycle;

    \draw[fill=magenta!20, opacity=.7] (2,-23) rectangle (3,-22);
    \node[anchor=west] at (3.5,-22.5) {\footnotesize qwen2.5-vl-72b};

\end{tikzpicture}
\caption{Per-task performance profiles by model}
\label{fig:Task-Model-Radar}
\end{subfigure}
\caption{(a) Model-level answer–time distributions (log scale). (b) Radar chart of per-task performance profiles by model across the seven Spatial-CAPTCHA task types. Profiles reveal task-specific strengths and weaknesses with little consistent coupling to latency.}
\label{fig:answer-response-times}
\end{figure*}

==> Figures/fig_difficulty_levels.tex <==

\begin{figure}[htbp]
\centering
\begin{subfigure}[c]{0.48\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=4pt,
    enlarge x limits=0.18,
    enlarge y limits={upper,value=0.2},
    ylabel={Score},
    symbolic x coords={o4-mini, Gemini-Pro, GPT-4o, Qwen2.5-VL, Phi-4, Gemini-Flash},
    xtick=data,
    ymin=0, ymax=60,
    axis y line*=left,
    axis x line*=bottom,
    legend style={
        at={(0.95,1.10)},
        anchor=north east,
        font=\scriptsize,
        draw=none,
        fill=white,
        fill opacity=0.8,
        text opacity=1,
        inner sep=4pt
    },
    legend columns=1,
    width=0.9\linewidth,
    height=0.7\linewidth,
    tick label style={font=\scriptsize},
    xticklabel style={rotate=60, anchor=north east}
]

\addplot+[style={fill=green!30}] coordinates {(o4-mini,59) (Gemini-Pro,55) (GPT-4o,73) (Qwen2.5-VL,82) (Phi-4,82) (Gemini-Flash,68)};
\addlegendentry{Easy Bin}

\addplot+[style={fill=yellow!40}] coordinates {(o4-mini,33) (Gemini-Pro,36) (GPT-4o,41) (Qwen2.5-VL,38) (Phi-4,32) (Gemini-Flash,31)};
\addlegendentry{Medium Bin}

\addplot+[style={fill=red!30}] coordinates {(o4-mini,27) (Gemini-Pro,24) (GPT-4o,8) (Qwen2.5-VL,6) (Phi-4,10) (Gemini-Flash,10)};
\addlegendentry{Hard Bin}

\addplot+[sharp plot, color=blue, mark=*, thick] coordinates {
    (o4-mini,30.95) (Gemini-Pro,30.92) (GPT-4o,26.10) (Qwen2.5-VL,24.00) (Phi-4,22.67) (Gemini-Flash,21.62)
};
\addlegendentry{Overall Score}

\node at (axis cs:o4-mini,33) {\scriptsize 31.0};
\node at (axis cs:Gemini-Pro,33) {\scriptsize 30.9};
\node at (axis cs:GPT-4o,28) {\scriptsize 26.1};
\node at (axis cs:Qwen2.5-VL,26) {\scriptsize 24.0};
\node at (axis cs:Phi-4,25) {\scriptsize 22.7};
\node at (axis cs:Gemini-Flash,24) {\scriptsize 21.6};

\end{axis}
\end{tikzpicture}
\caption{Model performance across difficulty levels}
\label{fig:subfig-spatial-scores}
\end{subfigure}
\hfill
\begin{subfigure}[c]{0.48\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar stacked,
    bar width=16pt,
    ymin=0, ymax=500,
    ylabel={Count},
    width=0.9\linewidth,
    height=0.85\linewidth,
    enlargelimits=0.15,
    % axis x line=bottom,
    % axis y line=left,
    symbolic x coords={SP, SO, MOR, SV},
    xtick=data,
    tick label style={font=\scriptsize},
    xticklabel style={rotate=60, anchor=north east},
    legend style={
        at={(0.01,0.99)},
        anchor=north west,
        font=\scriptsize,
        draw=none,
        fill=white,
        fill opacity=0.8
    },
    legend cell align={left},
    nodes near coords,
    nodes near coords align={center},
    every node near coord/.append style={font=\tiny,text=black},
    point meta=explicit symbolic,
]

\addplot+[ybar, fill=green!30] coordinates {
  (SP,6) [6]
  (SO,8) [8]
  (MOR,7) [7]
  (SV,7) [7]
};
\addlegendentry{Easy}

\addplot+[ybar, fill=yellow!40] coordinates {
  (SP,74) [74]
  (SO,166) [166]
  (MOR,187) [187]
  (SV,178) [178]
};
\addlegendentry{Medium}

\addplot+[ybar, fill=red!30] coordinates {
  (SP,70) [70]
  (SO,126) [126]
  (MOR,256) [256]
  (SV,115) [115]
};
\addlegendentry{Hard}

\end{axis}
\end{tikzpicture}
\caption{Difficulty distribution within spatial ability categories}
\label{fig:subfig-sc-vs-wsc}
\end{subfigure}

\caption{Spatial reasoning performance visualisation.}
\label{fig:spatial-overall-figure}
\end{figure}
